$R^3$: Reverse, Retrieve, and Rank for Sarcasm Generation with Commonsense Knowledge

We propose an unsupervised approach for sarcasm generation based on a non-sarcastic input sentence. Our method employs a retrieve-and-edit framework to instantiate two major characteristics of sarcasm: reversal of valence and semantic incongruity with the context which could include shared commonsense or world knowledge between the speaker and the listener. While prior works on sarcasm generation predominantly focus on context incongruity, we show that combining valence reversal and semantic incongruity based on the commonsense knowledge generates sarcasm of higher quality. Human evaluation shows that our system generates sarcasm better than human annotators 34% of the time, and better than a reinforced hybrid baseline 90% of the time.

==> comments.tex <==
% \violet{
% \begin{enumerate}
%     \item motivate the generation task by tying it to downstream applications of chatbot, or creative generation (slogans?)
%     \item list the challenges of this task (why is it hard?), this can motivate some of our model choice like the commonsense, negation, and NLI
%     \item introduce our solution: it's an \textit{unsupervised} method motivated by previous studies about sarcasm, like people studied the importance of NLI, negation, etc. so we add all those component.
%     \item list of contribution.
% \end{enumerate} }
% \sarik{
% The introduction is too length. My suggestions:
% \begin{enumerate}
%     \item First start with a definition of sarcasm in one or two sentences. 
%     \item Then talk about importance of sarcasm generation and its usecase in downstream tasks.
%     \item In the last paragraph, mention that your model outperforms SOTA in sarcasm generation (it can be one of the bullet points in the list of contributions) and move the improvement percentages into abstract.
% \end{enumerate} }
% The use of figurative language such as sarcasm is very familiar on social media-platform such as Twitter. Recognition of sarcasm is critical to understand people's actual sentiments and beliefs \cite{whocares} and in the last decade, automatic recognition of sarcasm has received a lot of attention in NLP research. In sarcastic utterances, the speakers typically mean the opposite of what they say. For instance, the utterance \textit{I love waiting at the doctor's office for hours} is sarcastic, expressing a negative sentiment toward the situation of \textit{waiting
% for hours at the doctor's office,} even if the speaker uses positive sentiment word such as \textit{love}.

 %Most research on sarcasm has focused on the task of \textit{Sarcasm Detection} treating it as a general text classification task using either the
% utterance in isolation or adding contextual information such as conversation context, author context, visual context, or cognitive features \cite{sarc1, sarc3,sarc4,sarc5,sarc6,sarc7,sarc8,sarc9,sarc10,sarc11}. 

%  we argue, besides \textit{sarcasm detection}, being able to \textit{generate sarcasm} will be a step forward in creative text generation

% There has been very few efforts towards automatic
% sarcasm generation hoewver where the generation is conditioned on a literal input sentence as shown in Table \ref{table:example1}.
% % also an important subtask of sarcasm research.
%  %DG - this needs a better sentence.

%Sarcasm is defined as an intensive, ironic construct that is intended to express contempt or ridicule\footnote{https://www.thefreedictionary.com/Sarcasm}.

% \violet{You motivate the problem as ``sarcasm exists in many places, previous work mainly focus on sarcasm detection, but we focus on generation.'' I think a better motivation would be: sarcasm generation is important and challenging, its success has high social impact, so we want to work on this problem.}

% \Smara{This introduction is too long, and the message gets lost. I can take a pass at it on Friday.I would refrain from using buzzwords such as strongAI/ Intro paragraph reads a bit like Mishra's first part and also his use of strong AI. } 

==> introduction_TC.tex <==
\section{Introduction} \label{section:introduction}
Social media has stimulated the production of user-generated content that contains figurative language use such as sarcasm. Recognizing sarcasm is critical for understanding people’s actual sentiments and beliefs \cite{whocares}. For instance, the utterance \textit{I love waiting at the doctor’s office for hours} is sarcastic, expressing a negative sentiment toward the situation of \textit{waiting
for hours at the doctor’s office,} even if the speaker uses positive sentiment word such as \textit{love}.

\newcite{sardef1} define Sarcasm as a type of interactional phenomenon with specific perlocutionary effects on the hearer such as to break their pattern of expectation. Sarcasm is also defined as an intensive, ironic construct that is intended to express contempt or ridicule \footnote{https://www.thefreedictionary.com/Sarcasm}. As it is often linked with intelligence, creativity, and wit, being able to generate Sarcasm is a step forward in creative text generation.

\begin{table}[]
\centering
\begin{tabular}{|l|}
\hline
I hate getting sick from fast food.                                                                                                                \\ \hline
\begin{tabular}[c]{@{}l@{}}Shout out to the McDonalds for \\giving me  bad food and making me \\sick right before  work in two hours.\end{tabular} \\ \hline
\end{tabular}
\caption{Table showing a literal or non sarcastic input sentence on the top and a human generated sarcastic version of the same}
\label{table:example1}
\end{table}

Generating content that is novel or creative is a key requirement in many natural language generation tasks such as poetry generation \cite{poetry1, poetry2}, story generation \cite{story1,story2}, pun generation \cite{pun1,pun2} etc. In this paper, we explore creative generation with a focus on sarcasm. Generating Sarcasm effectively can be useful to downstream applications such as conversation systems making them sound more natural,intriguing and human like.

Current approaches to text generation require huge amount of training data, but there are no such large corpus of sarcasm. Even in the presence of such a corpus, learning the distribution of existing data and sampling from it is unlikely to lead to truly novel and creative sentences. Creative composition requires deviating from the norm (i.e training samples) , whereas standard generation approaches seek to mimic the norm.

Most research on Sarcasm has focused on the task of \textit{Sarcasm Detection} treating it as a binary classification task using either the
utterance in isolation or adding contextual information such as conversation context, author context, visual context, or cognitive features \cite{sarc1, whocares, sarc3,sarc4,sarc5,sarc6,sarc7,sarc8,sarc9,sarc10,sarc11,sarc12}.There has been very few efforts towards automatic
sarcasm generation where the generation is conditioned on a literal input sentence as shown in Table \ref{table:example1}.

For Sarcasm speakers often rely on un-uttered knowledge such as mutually shared information or world knowledge.The human brain excels at understanding such implicit meanings, as people learn from experiences and feel certain emotions based on appraisals and inferences from related experiences. Computers, by contrast, lack such world
knowledge and can only rely on what they have learned from specific data.This motivates us to put CommonSense knowledge as the principle for guiding our Sarcasm generation approach.

Prior work on Sarcasm generation \cite{abhijit} has mostly focused on semantic incongruity in terms of contrasting sentiments.However for effective generation of Sarcasm we need to rely on various linguistic strategies as pointed out in \cite{phrasing}.To this end we build an end to end retrieval based generation framework where given a non sarcastic utterance as an input we generate a sarcastic version. In doing so we make use of 
\begin{itemize}
    \item \textbf{Lexical antonyms} and \textbf{Negation}
    \item \textbf{Pragmatic Inference} from a pre-trained language model fine-tuned on ConceptNet \cite{conceptnet} called COMET\cite{comet}
    \item Automatic way to measure \textbf{Semantic Incongruity} by relying on Contradiction scores obtained from a model trained on The Multi-Genre NLI Corpus \cite{multinli}
\end{itemize} 
We test our approach on 150 non sarcastic utterances randomly sampled from existing data sets.For qualitative evaluation, we consider the human judgment of Sarcastic intensity, Creativity, Humor and Grammaticality
of the generated sentences.  Human evaluation shows that our system generates better sarcasm  34 percent of the time compared to humans , and 89.3 percent times compared to a recent state of the art. We also present a thorough ablation of various components of our system further demonstrating that a system that incorporates all the strategies is the best one.





